Neural Text Summarization: A Critical Evaluation

Text summarization aims at compressing long documents into a shorter form that conveys the most important parts of the original document. Despite increased interest in the community and notable research effort, progress on benchmark datasets has stagnated. We critically evaluate key ingredients of the current research setup: datasets, evaluation metrics, and models, and highlight three primary shortcomings: 1) automatically collected datasets leave the task underconstrained and may contain noise detrimental to training and evaluation, 2) current evaluation protocol is weakly correlated with human judgment and does not account for important characteristics such as factual correctness, 3) models overfit to layout biases of current datasets and offer limited diversity in their outputs.

==> 3-related-work.tex <==
\section{Related Work}

% \subsubsection*{Other corpora}
% \paragraph*{AMI}~\citep{Carletta:05} is a set of transcripts of real and staged office meetings.
% The dataset contains 138 examples which translate to 100h of recordings.
% Each transcript is associated with with an abstractive and extractive summary written by annotators according to strict guidelines.


% \paragraph*{Reddit Personal Narratives}~\citep{McKeown:17} is a data collection scraped from Reddit.
% Articles represent personal narratives written by the users written in response to 19 different prompts (questions).
% Given the source of the data, the articles use mostly informal language.
% Each article comes with an aligned abstractive and extractive summary.
% In addition to alignment information, abstractive summaries are also annotated with phrase-level rewrite operations generated by humans.
% Both the summaries and other annotation data was collected by the authors of the dataset through MTurk.
% The dataset has a total of 1088 examples.




==> 8-background.tex <==
\section{Background} \label{sec:related-work}

\subsection{Datasets}
In the following subsection we briefly describe the available large scale datasets for text summarization.

\paragraph*{Gigaword}~\citep{Graff:03} is a collection of news data coming from different domestic and international news sources.
The articles in the dataset cover a mix of topics and each article is associated with a short, single sentence headline.
The dataset was not originally designed for the task of summarization, but naively adapted to its needs.
The short, single-sentence headers of each article are treated as target summaries for articles.
In its original version, the dataset contained 4.1M article-headline pairs. 
Since its introduction, the dataset has been extended multiple-times, where each extension added news sources and articles following time spans.
The latest version contains 9.8M documents acquired from 7 news sources. 
Despite its large number of articles, the major limitation of the dataset is the short length of target summaries.
The data was previously used for headline generation \citep{Takase:16} and single-sentence summarization \citep{Rush:15, Chopra:16}. 

\paragraph*{NYT}~\citep{Sandhaus:08} is a collection of articles from the New York Times magazine. 
The articles were published between 1987 and 2007 and cover a broad range of topics.
The dataset contains a total of 1.8M articles, out of which 650k have associated abstracts written by library scientists.
280k articles from the dataset come with an additional, short summary that was used as a snippet in the digital edition of the magazine.
The articles in the dataset lean towards long-form essays, which makes the important information more spread out across the text, instead of being primarily biased towards the beginning.
The dataset is available for a licensing fee.
The dataset has been primarily used for extractive summarization \citep{Hong:14, Li:16} and phrase importance prediction \citep{Yang:14, Nye:15}.

\paragraph*{CNN/DailyMail}~\citep{Nallapati:16} is a set of news articles from the online editions of CNN and DailyMail services. 
The dataset contains 310k articles covering a broad range of topics, ranging from politics to sports.
Each article is associated associated with a multi-sentence summary that was constructed by concatenating article highlights provided as bullet points.
Originally, the dataset was introduced by \cite{Hermann:15} in the form of Cloze style question-answer pairs for machine reading comprehension. 
The dataset is available in two version, anonymized, where entity names are replaced with a special \texttt{@entity} token, and deanonimized, where entity names are not processed in any way.
The adapted version of the CNN/DailyMail dataset has been used for both extractive \citep{Dong:18, Wu:18, Zhao:18} and abstractive \citep{See:17, Paulus:17, Kryscinski:18} summarization.

\paragraph*{Newsroom}~\citep{Grusky:18} is a collection of news articles sourced from 38 major online news outlets.
Articles were published between 1998 and 2017 and cover a broad range of topics, including politics, finance, and sports.
The dataset contains a total of 1.3M articles, each coming with a single, multi-sentence summary.
Target summaries in the dataset were written by journalists and newsroom editors to be displayed as article snippets on social media platforms.
The large number of data sources is reflected in a variety of writing styles and different levels of abstraction of summaries.
Examples in the dataset are organized into groups based on the level of abstraction of target summaries.
The dataset was released together with a leaderboard and held-out testing split.
At the time of writing this paper, the Newsroom dataset is the largest multi-sentence dataset for text summarization.

\paragraph*{XSum}~\citep{Kim:18} is a collection of news articles coming from the BBC website.
Articles were collected between 2010 and 2018, each article is associated with one, single-sentence summary.
There are a total of 225k articles in the dataset.
Given that the articles come from a single news outlet, they are written in a similar style and have provided summaries have a equal level of abstraction.
The authors also showed that the target summaries are highly abstractive, preventing models from simply extracting the leading sentences from the source document.

\paragraph*{WikiHow}~\citep{Koupaee:18} is a collection of articles from the WikiHow knowledge base.
WikiHow contains instructions for performing procedural, multi-step tasks covering various areas, from arts to electronics. 
The instructions in the knowledge base are written in a collaborative fashion by multiple authors, increasing the variety of writing styles.
Each training example is a single-step extracted from the instruction.
The article is a detailed explanation of how to correctly perform the step, while the target summary is a short description of the step.
The dataset has a total of 230k examples and covers both single, and multi-sentence summaries.
Authors showed, that the summaries are highly abstractive, and the Lead-3 baseline does not perform well on the dataset.

\paragraph*{Reddit TIFU}~\citep{Kim:18} is a collection of posts scraped from the discussion forum Reddit.
All articles were collected from the subreddit \textit{TIFU}, where users post their daily stories and ask other users for opinions.
The rules of the subreddit require users to include a summary (\textit{TL;DR}) alongside their story.
Collected articles were written between 2013 and 2018, each article in the dataset comes with one associated summary.
The dataset was released in two versions, \textit{TIFU-short} with 80k examples, where summaries are written in a short, headline-like fashion, and \textit{TIFU-long} with 42k examples, where summaries span over multiple sentences.
Given the nature of the source, the articles reflect different writing styles and the language is mostly casual.
Collected data has weak Lead-3 bias and strong abstractiveness.

\subsection{Evaluation Metrics}
This section briefly describes the available evaluation methods introduced for the task of summarization.

\paragraph*{Pyramids}~\citep{Nenkova:04} is a semi-automatic evaluation method that compares summaries based shared content units.
The method requires multiple reference summaries and uses human annotators to extract summary content units (SCUs).
Discovered SCUs are organized in a pyramid, where each unit is assigned a weight that is proportional to the number of occurrences in different summaries.
To evaluate summarization models, annotators extract SCUs from the candidate summary and a scores is calculated based on the SCU overlap between the generated summary and the Pyramid.
To limit the human effort required to evaluate new models, an updated version of Pyramids was introduced by \citet{Passonneau:13}. 
The new version assumed only annotations of the reference summaries and automatically computed similarities between model generated outputs and content units using word embeddings.

\paragraph*{ROUGE}~\citep{Lin:04} is an automatic evaluation toolkit offering a set of metrics based on an exact $n$-gram overlap between the candidate and reference summaries. 
The simplest metrics measure the overlap of consecutive sequences of tokens of a predefined size, e.g. ROUGE-1 (unigrams), ROUGE-2 (bigrams).
The toolkit also offers more complex metrics that take into account the longest common subsequence of tokens, ROUGE-L(CS), and gaps between matched tokens (skipgrams), ROUGE-SU.
In its original form, the ROUGE metrics were based on the recall measure, but they were later extended with precision and $F_1$ measures to handle cases where the reference and candidate sequences were of varying length.
Despite its simplicity, ROUGE-1, ROUGE-2, and ROUGE-L(CS) $F_1$-scores have become the standard evaluation metric for summarization models.

\paragraph*{ParaEval}~\citep{Zhou:06} is an automatic evaluation metric based on a three-tier comparison strategy, that aims at handling cases where generated summaries are abstractive.
In the highest tier, the method performs an optimal search to find multi-word paraphrase matches between the candidate and reference summaries.
Unmatched subsequences are passed to the middle-tier, where a greedy search is conducted to find single-word synonym matches.
The third and lowest-tier handles any left out tokens and looks for exact lexical matches in a style similar to ROUGE.
Paraphrase matches in the highest and middle tier are done based on an paraphrase table built from a bilingual parallel corpus with the help of a Machine Translation system.
Despite promising results shown by the authors the evaluation scripts were not made publicly available.

\paragraph*{ROUGE-WE}~\citep{Ng:15} is an automatic evaluation metric that aims to address the shortcomings of exact lexical matching used in the ROUGE toolkit.
Authors proposed replacing the $n$-gram overlap with a soft similarity measure between words in the target and candidate summaries.
ROUGE-WE represents each word in both of the summaries with their word2vec representations \citep{Mikolov:13} and computes the similarity between the sequences based on their cosine distances.
The method allows computing scores for $n$-grams of any size by composing embeddings of phrases out of embeddings of single words in a multiplicative fashion.

\paragraph*{ROUGE 2.0}~\citep{Ganesan:18} is an automatic evaluation matric that extends the original ROUGE with support for synonym matching and topic-specific evaluation.
To support synonym matching, the authors leverage synonym dictionaries, such as WordNet.
When measuring $n$-gram overlap, the metric not looks for exact matches, but also considers synonms.
Topic-specific evaluation allows to measure specific dimensions of the summary. 
Using a POS Tagger, ROUGE 2.0 can be set to measure only the overlap of specific parts-of-speech, such as verbs or nouns, which can be valuable when evaluating certain domains.

\paragraph*{Human Studies} are often used alongside automatic metrics, such as ROUGE, to evaluate the quality of generated outputs.
Human workers are employed on a per-task basis through popular crowdsourcing platforms, such as Amazon Mechanical Turk or CrowdFlower. 
Common evaluation methods use the Likert scale, with values between 1 and 5, and ask the annotators to evaluate the summaries across distinct dimensions, such as \textit{Readability} and \textit{Relevance}. 
Another popular evaluation method uses pairwise comparisons between models, where the annotators are simply asked to choose the best from a fixed set of summaries across the mentioned dimensions.
Despite the easy and relatively cheap access to thousands of human annotators, crowdsourced human studies are known to yield noisy measurements. 
To ensure high quality, reliable results, such studies require detailed experiment planning and data curation.

==> custom-commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

